Informative co-data learning for high-dimensional Horseshoe regression

High-dimensional data often arise from clinical genomics research to infer relevant predictors of a particular trait. A way to improve the predictive performance is to include information on the predictors derived from prior knowledge or previous studies. Such information is also referred to as ``co-data''. To this aim, we develop a novel Bayesian model for including co-data in a high-dimensional regression framework, called Informative Horseshoe regression (infHS). The proposed approach regresses the prior variances of the regression parameters on the co-data variables, improving variable selection and prediction. We implement both a Gibbs sampler and a Variational approximation algorithm. The former is suited for applications of moderate dimensions which, besides prediction, target posterior inference, whereas the computational efficiency of the latter allows handling a very large number of variables. We show the benefits from including co-data with a simulation study. Eventually, we demonstrate that infHS outperforms competing approaches for two genomics applications.

==> MyDef/def_callig.tex <==
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% CALLIGRAPHIC SYMBOLS
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
\def\calC{\mbox{\boldmath ${\cal C}$}} 
\def\calT{\mbox{\boldmath ${\cal T}$}}
\def\calU{\mbox{\boldmath ${\cal U}$}} 
\def\calK{\mbox{\boldmath ${\cal K}$}}
\def\calA{\mbox{\boldmath ${\cal A}$}} 
\def\calD{\mbox{\boldmath ${\cal D}$}}
\def\calE{\mbox{\boldmath ${\cal E}$}}

==> MyDef/def_color.tex <==
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% COLORS
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
\definecolor{darkross}{rgb}{0.008,0.412,0.471}
\definecolor{middleross}{rgb}{0.012,0.580,0.663}
\definecolor{lightross}{rgb}{0.016,0.749,0.855}
\definecolor{darkblue}{rgb}{0.067,0.008,0.471}
\definecolor{middleblue}{rgb}{0.094,0.012,0.663}
\definecolor{lightblue}{rgb}{0.122,0.016,0.855}
\definecolor{darkpurple}{rgb}{0.471,0.008,0.412}
\definecolor{middlepurple}{rgb}{0.663,0.012,0.580}
\definecolor{lightpurple}{rgb}{0.855,0.016,0.749}
\definecolor{darkbrown}{rgb}{0.471,0.067,0.008}
\definecolor{middlebrown}{rgb}{0.663,0.094,0.012}
\definecolor{lightbrown}{rgb}{0.855,0.122,0.016}
\definecolor{darkolive}{rgb}{0.412,0.471,0.008}
\definecolor{middleolive}{rgb}{0.580,0.663,0.012}
\definecolor{lightolive}{rgb}{0.749,0.855,0.016}
\definecolor{darkgreen}{rgb}{0.008,0.417,0.067}
\definecolor{middlegreen}{rgb}{0.012,0.663,0.094}
\definecolor{lightgreen}{rgb}{0.016,0.855,0.122}
\definecolor{darkocre}{rgb}{0.471,0.298,0.008}
\definecolor{middleocre}{rgb}{0.663,0.420,0.012}
\definecolor{lightocre}{rgb}{0.855,0.541,0.016}
%
\def\colorred{\color{red}}
\def\colorblue{\color{middleblue}}
\def\colorgreen{\color{green}}
\def\coloryellow{\color{yellow}}

\def\colordarkross{\color{darkross}}
\def\colordarkblue{\color{darkblue}}
\def\colorlightblue{\color{lightblue}}
\def\colorlightbrown{\color{lightbrown}}
\def\colordarkgreen{\color{darkgreen}}

==> MyDef/def_letters_acc.tex <==
\def\ac{\`a}
\def\ec{\`e}
\def\uc{\`u}
\def\oc{\`o}
\def\ic{\`i}

\def\acsp{\`a }
\def\ecsp{\`e }
\def\ucsp{\`u }
\def\ocsp{\`o }
\def\icsp{\`i }

\def\qmo{``}
\def\qmc{''}
\def\qmcsp{'' }

==> MyDef/def_letters_b.tex <==
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% LETTERS
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}} 
\def\bi{\mathbf{i}} 
\def\bh{\mathbf{h}}
\def\bp{\mathbf{p}} 
\def\bP{\mathbf{P}}
\def\bff{\mbox{\boldmath $f$}} 
\def\bl{\mbox{\boldmath $l$}}
\def\bJ{\mathbf{J}}
\def\bw{\mathbf{w}}
\def\bL{\mathbf{L}}
\def\br{\mathbf{r}}
\def\bu{\mathbf{u}} 
\def\bt{\mathbf{t}}
\def\by{\mathbf{y}} 
\def\bY{\mathbf{Y}}
\def\0{\mbox{\bf{0}}}
\def\bs{\mathbf{s}}
\def\bS{\mathbf{S}}
\def\bI{\mathbf{I}}
\def\be{\mathbf{e}}
\def\bz{\mathbf{z}}
\def\bZ{\mathbf{Z}}
\def\bC{\mathbf{C}} 
\def\bM{\mathbf{M}}
\def\bc{\mathbf{c}} 
\def\bT{\mathbf{T}}
\def\bW{\mathbf{W}} 
\def\bN{\mathbf{N}} 
\def\bR{\mathbf{R}}
\def\bG{\mathbf{G}} 
\def\bX{\mathbf{X}} 
\def\bx{\mathbf{x}}
\def\bO{\mathbf{0}}
\def\bg{\mathbf{g}}
\def\bv{\mathbf{v}}%
\def\bw{\mathbf{w}}%
\def\bq{\mathbf{q}}
\def\bQ{\mathbf{Q}}
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% CAPITAL LETTERS
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
\def\bA{\mathbf{A}}
\def\bE{\mathbf{E}}
\def\bK{\mathbf{K}}
\def\bQ{\mathbf{Q}}
\def\bH{\mathbf{H}}
\def\bF{\mathbf{F}}
\def\bB{\mathbf{B}}
\def\bD{\mathbf{D}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}} 

==> MyDef/def_theorem.tex <==
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% THEOREMS AND PROOFS
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{property}{Property}[section]
%\newtheorem{algorithm}{Algorithm}[section]
\newtheorem{example}{Example}[section]

==> MyDef/def_virg.tex <==
\def\qmo{``}
\def\qmc{''}
\def\qmcsp{'' }
